Reinforced Sequential Decision-Making for Sepsis Treatment: The POSNEGDM Framework with Mortality Classifier and Transformer

Sepsis, a life-threatening condition triggered by the body's exaggerated response to infection, demands urgent intervention to prevent severe complications. Existing machine learning methods for managing sepsis struggle in offline scenarios, exhibiting suboptimal performance with survival rates below 50%. This paper introduces the POSNEGDM -- ``Reinforcement Learning with Positive and Negative Demonstrations for Sequential Decision-Making" framework utilizing an innovative transformer-based model and a feedback reinforcer to replicate expert actions while considering individual patient characteristics. A mortality classifier with 96.7\% accuracy guides treatment decisions towards positive outcomes. The POSNEGDM framework significantly improves patient survival, saving 97.39% of patients, outperforming established machine learning algorithms (Decision Transformer and Behavioral Cloning) with survival rates of 33.4% and 43.5%, respectively. Additionally, ablation studies underscore the critical role of the transformer-based decision maker and the integration of a mortality classifier in enhancing overall survival rates. In summary, our proposed approach presents a promising avenue for enhancing sepsis treatment outcomes, contributing to improved patient care and reduced healthcare costs.

==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

	
	
\begin{table*}[]
\centering
\scalebox{0.85}{
\begin{tabular}{|c|c|ccl|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & \multicolumn{2}{c}{Action Prediction Accuracy} & \\ \hline
 Method & Parameter & \multicolumn{1}{c|}{Positive Trajectories} & Negative Trajectories &  \\ \hline
Decision Transformer \citep{b1} & $-$ & \multicolumn{1}{c|}{0.94} & 0.9063 &  \\ \hline
Behavioral Cloning \citep{b16} & $-$ & \multicolumn{1}{c|}{0.945} & 0.92 &  \\ \hline
% Behaviour cloniong &  & \multicolumn{1}{c|}{} &  &  \\ \hline
% GAIL (After the first draft) &  & \multicolumn{1}{c|}{} &  &  \\ \hline
\multirow{4}{*}{\name (Ablation: next state prediction)} & $\lambda$ = 0.1 & \multicolumn{1}{c|}{0.9379} & 0.8063 &  \\ \cline{2-5} 
 & $\lambda$ = 1 & \multicolumn{1}{c|}{\textbf{0.9353}} & \textbf{0.797} &  \\ \cline{2-5} 
 & $\lambda$ = 5 & \multicolumn{1}{c|}{0.944} & 0.8326 &  \\ 
%\cline{2-5} 
 & $\lambda$ = 10 & \multicolumn{1}{c|}{0.944} & 0.8725 &  \\ \hline
\multirow{4}{*}{\name (Ablation: negative trajectory divergence)} & $\beta$ = -5 & \multicolumn{1}{c|}{0.1016} & 0.014 &  \\ \cline{2-5} 
 & $\beta$ = 1 & \multicolumn{1}{c|}{0.9244} & 0.8892 &  \\ \cline{2-5} 
 & $\beta$ = 5 & \multicolumn{1}{c|}{0.8499} & 0.6632 &  \\ \cline{2-5} 
 & $\beta$ = 10 & \multicolumn{1}{c|}{0.8336} & 0.7165 &  \\ \hline
\end{tabular}
}
\caption{Experimental Results}
\label{tab:results}
\end{table*}

